MMT/Binospec Spectroscopic Survey of Two $z\sim$ 0.8 Galaxy Clusters in the Eye of Horus Field

The discovery of the Eye of Horus (EoH), a rare double source-plane lens system ($z_{\rm lens}=$ 0.795; $z_{\rm src}=$ 1.302 and 1.988), has also led to the identification of two high-redshift ($z_{\rm phot}\sim$ 0.8) galaxy clusters in the same field based on the subsequent analysis of the Subaru/Hyper Suprime-Cam (HSC) optical and XMM-Newton X-ray data. The two brightest cluster galaxies (BCGs), one of which is the lensing galaxy of the EoH, are separated by only $\sim$100$"$ ($=$ 0.75 Mpc $<$ $r_{200}$) on the sky, raising the possibility that these two clusters may be physically associated. Here, we present a follow-up optical spectroscopic survey of this EoH field, obtaining 218 secure redshifts using MMT/Binospec. We have confirmed that there indeed exist two massive ($M_{\rm dyn}$ $>$ $10^{14}$ M$_\odot$) clusters of galaxies at $z$ $=$ 0.795 (the main cluster) and at $z=0.769$ (the NE cluster). However, these clusters have a velocity offset of $\sim$4300 km s$^{-1}$, suggesting that this two-cluster system is likely a line-of-sight projection rather than a physically-related association (e.g., a cluster merger). In terms of the properties of cluster-member galaxies, these two $z\sim0.8$ clusters appear well-developed, each harboring an old (age $=$ 3.6-6.0 Gyr) and massive ($M_\mathrm{*}$ $=$ 4.2-9.5 $\times$ $10^{11}$ M$_\odot$) BCG and exhibiting a well-established red sequence (RS). This study underscores the importance of conducting a spectroscopic follow-up for high-redshift cluster candidates because RS-based cluster selections are susceptible to such a projection effect in general.

==> show_2dspec_figset_to_ApJ.tex <==
% Example figure in paper
\clearpage
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth, height=0.96\textheight, keepaspectratio]{figures_spec2d/1d+2dspec_01.jpg}
    \caption{Galaxy Spectra of Slit~\#1--8.}
\end{figure*}

% Set of figures in online ApJ
\figsetstart

\figsetnum{8}
\figsettitle{Galaxy Spectra}

\figsetgrpstart
\figsetgrpnum{8.1}
\figsetgrptitle{Slit~\#1--8}
\figsetplot{figures_spec2d/1d+2dspec_01.pdf}
\figsetgrpnote{}
\figsetgrpend


\figsetend
